Twisted relative Cuntz-Krieger algebras associated to finitely aligned higher-rank graphs

To each finitely aligned higher-rank graph $\Lambda$ and each $\mathbb{T}$-valued 2-cocycle on $\Lambda$, we associate a family of twisted relative Cuntz-Krieger algebras. We show that each of these algebras carries a gauge action, and prove a gauge-invariant uniqueness theorem. We describe an isomorphism between the fixed point algebras for the gauge actions on the twisted and untwisted relative Cuntz-Krieger algebras. We show that the quotient of a twisted relative Cuntz-Krieger algebra by a gauge-invariant ideal is canonically isomorphic to a twisted relative Cuntz-Krieger algebra associated to a subgraph. We use this to provide a complete graph-theoretic description of the gauge-invariant ideal structure of each twisted relative Cuntz-Krieger algebra.

==> chapter6_Conclusion.tex <==
\chapter{Conclusion} %
\label{chptr:conclusion}

Now that we understand the gauge-invariant ideal structure of $C^*(\Lambda,c;\mathcal{E})$, we would like to know when every ideal of $C^*(\Lambda,c;\mathcal{E})$ is gauge-invariant, and when $C^*(\Lambda,c):=C^*(\Lambda,c;\FE(\Lambda))$ is simple.

In (Section 7, \cite{S20062}), Sims identifies a necessary condition that $\Lambda$ must satisfy so that all the ideals of $C^*(\Lambda,\hat 1)$ are gauge-invariant. In (Section 8, \cite{S20062}), Sims shows that if $\Lambda$ satisfies condition (C) then $C^*(\Lambda,\hat 1)$ is simple if and only if $\Lambda$ is \emph{cofinal} (Definition 8.4, \cite{S20062}). Corollary 8.2 of \cite{KPS2012b} shows that if $\Lambda$ is row-finite and has no sources, then the result also holds for $C^*(\Lambda,c)$, where $c$ is an arbitrary 2-cocycle. The same should be true for finitely aligned $k$-graphs. So the simplicity of $C^*(\Lambda,\hat 1)$ implies the simplicity of $C^*(\Lambda,c)$, but not conversely.

Their is a unique $2$-graph $\Lambda$ with $1$-skeleton:
\begin{center}
\begin{tikzpicture}[scale=1.5]
\node (u) at (0,0) {$v$};
%
\draw[blue, -latex] (u.north west) .. controls +(-0.6, 0.6) and +(-0.6, -0.6) .. (u.south west) node[pos=0.5, left, black] {$e$};
%
\draw[red, -latex] (u.south east) .. controls +(0.6, -0.6) and +(0.6, 0.6) .. (u.north east) node[pos=0.5, right, black] {$f$};
\end{tikzpicture}
\end{center}
This $2$-graph doesn't satisfy condition (C). The map
\begin{equation}c_\theta (e^m f^n, e^p f^q)=e^{2 \pi i \theta np}\nonumber\end{equation}
is a 2-cocycle for each $\theta \in [0,1)$. The twisted Cuntz-Krieger algebra $C^*(\Lambda,c_\theta)$ is the universal $C^*$-algebra generated by two unitaries $u$ and $v$ satisfying
$$uv=e^{2\pi i \theta} v u.$$
That is, $C^*(\Lambda,c_\theta)$ is the rotation algebra $\mathcal{A}_\theta$. The rotation algebra $\mathcal{A}_\theta$ is simple if and only if $\theta$ is irrational. We would like to know conditions on $\Lambda$ and $c$ so that $C^*(\Lambda,c)$ is simple, and conversely. 
